Toward Separating QMA from QCMA with a Classical Oracle

QMA is the class of languages that can be decided by an efficient quantum verifier given a quantum witness, whereas QCMA is the class of such languages where the efficient quantum verifier only is given a classical witness. A challenging fundamental goal in quantum query complexity is to find a classical oracle separation for these classes. In this work, we offer a new approach towards proving such a separation that is qualitatively different than prior work, and show that our approach is sound assuming a natural statistical conjecture which may have other applications to quantum query complexity lower bounds.

==> sep.tex <==
\section{Our Separating Oracle}\label{sec:sep}

We now give our oracles which are conjectured to separate $\QMA$ from $\QCMA$. We will prove:

\begin{theorem}\label{thm:main}Assuming Conjecture~\ref{conj:main}, there is a classical oracle $\Os$ such that $\QMA^\Os\neq\QCMA^\Os$.
\end{theorem}
\begin{corollary}Assuming Conjecture~\ref{conj:stat}, there is a classical oracle $\Os$ such that $\QMA^\Os\neq\QCMA^\Os$.\end{corollary}

\noindent The rest of this section is devoted to the proof of Theorem~\ref{thm:main}.

\begin{proof}Since we assume Conjecture~\ref{conj:main} to be true, there exists functions $p,\epsilon,\delta,\gamma:\Z^+\rightarrow[0,1]$ and functions $N,k:\Z^+\rightarrow\Z^+$ such that (1) $p(n),\epsilon(n),\delta(n)\leq n^{-\omega(1)}$, (2) $N(n)\leq 2^{n^{O(1)}}$ (3) $k(n)\geq n^{\omega(1)}$, (4) $\gamma\geq n^{-O(1)}$, and (5) except with probability $\epsilon(n)$ over the choice of $S\gets\Bernoulli_{p(n)}^{N(n)}$, there exists a distribution $\Ds_S$ over pairs $(|\psi\rangle,U)$ such that:
	\begin{itemize}
		\item $U$ is a subset of $[N(n)]$, and the marginal distribution of $U$ is $k(n)$-wise uniform independent.
		\item $|\psi\rangle$ is a normalized superposition $\sum_{x\in S}\alpha_x|x\rangle$ over elements in $S$.
		\item Except with probability $\delta(n)$ over the choice of $(|\psi\rangle,U)\gets\Ds_S$, $\langle \hat{\psi}|\Pi_U |\hat{\psi}\rangle\geq \frac{1}{2}+\gamma(n)$.
	\end{itemize}
We will invoke the definition of $\QMA$ and $\QCMA$ with $a=1/2+\gamma(n)/2$ and $b=1/2+\gamma(n)$. Since $b-a=\gamma(n)/2$ is inverse polynomial, this is equivalent to the standard definition of $\QMA$ and $\QCMA$. Thus, a valid verifier will accept YES instances of size $n$ (given a correct witness) with probability at least $1/2+\gamma(n)$, and accept NO instances with probability at most $1/2+\gamma(n)/2$. We can always assume without loss of generality that there is, say, a fixed quadratic running time $t$ such that the running time of any $\QCMA$ verifier is bounded by $t(|x|+|w|)$ where $|x|$ is the instance length and $|w|$ is the witness length. This is accomplished by padding the witness length with 0's that just get ignored by the verifier. 

Our oracle $\Os$ will be the combination of oracles $S_n,U_n$ for each $n\in\Z^+$ where $S_n,U_n$ correspond to subsets of $[N(n)]$. In order to specify $S_n,U_n$, let $\Ts=(\Ts_i)_{i\in\Z^+}$ be some enumeration over all oracle-aided quadratic-time quantum algorithms. Let $q(n)$ be a sufficiently small super-polynomial function, which we will take as an upper bound on witness length. Let $Q(n)=q(n)^2$, which we take to be an upper bound on the number of queries when the witness length is at most $q(n)$. Let $v(n)$ be another super-polynomial. We will need the following constraints on $q,Q,v$:
\begin{align*}
	Q&\ll \gamma p^{-1/2}&
	v&\gg qQ^4\gamma^{-4}\\
	v&\ll \gamma N^{1/12}&
	Qk/v&\leq n^{-\omega(1)} 
\end{align*}

The above quantities can be satisfied for a sufficiently-small super-polynomial $q,v$ and for sufficiently large $n$. We now let $n_1$ be a sufficiently large constant such that all the inequalities above hold for $n\geq n_1$. We will place further lower-bounds on $n$ later in the proof. Let $n_i=O(q(n_{i-1})^3)$, which ensures that $\Ts_i$, on input instances of length $n_i$ and witnesses of length at most $q(n_i)$, has zero query mass on $S_{n'}$ or $U_{n'}$ for $n'\geq n_{i+1}$, simply because it cannot run in enough time to even produce a query of sufficient length.

We now describe our sets $S_n,U_n$. At the same time, we will also describe our language $\Language^\Os$. $\Language^\Os$ will be a subset of the strings $\{0^{n_i}\}_i$. For $n$ outside $\{n_i\}_i$, we set $S_n=U_n=\emptyset$. Then for each $n_ii$, $S_{n_i},U_{n_i}$ and the membership of $0^{n_i}$ in $\Language^\Os$ will be determined by the following loop. For $i=1,\cdots$ do the following:
\begin{enumerate}
	\item Sample $S\gets \Bernoulli_{p(n_i)}^{N(n_i)}$ and $(|\psi\rangle,U)\gets \Ds_{S}$. 
	\item Observe that $\Ts_i^\Os(0^{n_i},w)$ for $|w|\leq q(n_i)$ will only make queries to $S_n,U_n$ for $n < n_{i+1}$. Also, note that previous iterations of this loop have defined $S_n,U_n$ for all $n<n_{i+1}$, except for $n=n_i$. Let $\Os_i$ be the oracle containing the previously defined $S_n,U_n$, and which answers queries to $S_{n_i}$ with $S$ and queries to $U_{n_i}$ with $U$.
	\item Check if there is a witness $w_i$ of length at most $q(n_i)$ such that $\Ts_i^{\Os_i}(0^{n_i},w_i)$ accepts with probability at least $1/2+\gamma(n_i)$. 
	\item \label{step:yes} If there is \emph{no} such witness, set $S_{n_i}=S$ and $U_{n_i}=U$ and put $0^{n_i}$ in $\Language^\Os$. Move on to the next iteration of the loop.
	\item If there \emph{is} such a $w_i$, then we exclude $0^{n_i}$ from $\Language^\Os$. We also initialize a list $S'=\{\}$. Now repeat the following $v(n_i)$ times:
	\begin{itemize}
		\item Run $\Ts_i^{\Os_i}(0^{n_i},w_i)$ until a randomly chosen query and measure the query. 
		\item If the resulting string $y$ is a query to $S$, and moreover if the result of the query is that $y\in S$, then add $y$ to $S'$.
	\end{itemize}
	Now set $S_{n_i}=S'$ and $U_{n_i}=U$, and move on to the next iteration of the loop.
\end{enumerate}

\noindent We now prove that the $\Language^\Os$ constructed above in $\QMA^\Os\setminus\QCMA^\Os$ with positive probability.

\paragraph{$\Language^\Os\in\QMA$.} We first explain that $\Language^\Os\in\QMA$. Our verifier $V^\Os$ will work as follows. On input $x\in\{0,1\}^n$, if $x\neq 0^n$, $V^\Os$ will reject. If $x=0^n$, then $V^\Os$ will make a query to $S_n$ on the witness state $|\phi\rangle$ and measuring the output. If it accepts, then $V^\Os$ will apply the $\QFT$ to the witness state (which may have changed due to the measurement), and make a query to $U_n$, measuring the output. If both queries accept, then $V^\Os$ will output 1; if either measurement rejects, then $V^\Os$ will output 0.

To see that $V$ is correct, we first need the following, which is proved in Section~\ref{sec:missproof}:
\begin{lemma}\label{lem:pairwisesmall} If $U$ is sampled from a $k'$-wise uniform independent function and $S'$ is correlated to $U$ but has size at most $v$, then except with probability $2N^2\left(\frac{\sqrt{ek'}}{\epsilon\sqrt{N}}\right)^{k'}$ over the choice of $U,S'$, it holds that, for any normalized state $|\phi\rangle$ with support on $S'$, $\langle\hat{\phi}|\Pi_U|\hat{\phi}\rangle\leq 1/2+v\epsilon$, where $|\hat{\phi}\rangle=\QFT|\phi\rangle$.
\end{lemma}



\noindent We now analyze the behavior of $V$ by breaking into cases:
\begin{itemize}
	\item $x\in\{0,1\}^n\setminus\{0^n\}$. In this case, $x\notin\Language^\Os$ and $V^\Os$ rejects.
	\item $x=0^n$ but $n\neq n_i$ for any $i$. In this case, $x\notin\Language^\Os$, and since $S_n,U_n$ are empty $V^\Os$ rejects regardless of the witness state.
	\item $x=0^{n_i}$ and the construction of $\Os$ sets $S_{n_i}=S$ and $U_{n_i}=U$. In this case, $x\in\Language^\Os$. Moreover, if we set the witness $|\phi\rangle$ to be the state $|\psi\rangle$ generated along side $U$ by $\Ds_S$, the guarantee of Conjecture~\ref{conj:main} is exactly that, with overwhelming probability over the choice of $S,U,|\psi\rangle$, $V^\Os$ accepts with probability at least $1/2+\gamma(n)$.
	\item $x=0^{n_i}$ and the construction of $\Os$ sets $S_{n_i}=S'$ and $U_{n_i}=U$. In this case, we observe that $S'$ can have size mo more than $v(n_i)$. Moreover, the highest probability witness states will always have support on $S'$, since the first step of $V^\Os$ is to project out all points not in $S'$. We then invoke Lemma~\ref{lem:pairwisesmall} with $\epsilon=\gamma/3v$ to see that, except with probability at most $G:=2N^2\left(\frac{3v\sqrt{ek'}}{\gamma\sqrt{N}}\right)^{k'}$ over the choice of $U$, $V^\Os$ accepts with probability at most $1/2+\gamma/3< 1/2+\gamma/2$, no matter what $S'$ is. Setting $k'=5$ and using that $v\leq \gamma N^{1/12}$ we have that $G=O(N^{1/12})$, which is negligible.
\end{itemize}

Note that for each $n_i$ the above may fail to construct $\Os,\Language^\Os$ such that $V^\Os$ accepts $\Language^\Os$. However, we showed that there is a function $f(n)\leq n^{-\omega(1)}$ such that this probability is bounded by $f(n_i)$. We then use that $\sum_{n'\geq n} f(n')\leq n^{-\omega(1)}$ for any negligible function $f$, to bound the probability of any failure among all the $n_i$ is at most negligible in $n_1$. We will therefore set $n_1$ large enough so that this probability is at most $1/3$.



\paragraph{$\Language^\Os\notin\QCMA$.} We now show that $\Language^\Os\notin\QCMA$. Suppose towards contradiction that $\Language^\Os\in\QCMA$. By our enumeration $\Ts$ over quantum algorithms, this means there is an $i$ such that $\Ts_i$ decides $\Language^\Os$ with polynomial-length witnesses. Consider $\Ts_i$ with instance $x=0^{n_i}$. If $x\in\Language^\Os$, then by construction there does not exist a string $w_i$ of polynomial length such that $\Ts_i^{\Os_i}(0^{n_i},w_i)$ accepts with probability at least $1/2+\gamma(n_i)$. But for $x\in\Language^\Os$, $\Os$ and $\Os_i$ agree on all points queried by $\Ts_i$, meaning there is also no string $w_i$ of polynomial length such that $\Ts_i^{\Os}(0^{n_i},w_i)$ accepts with probability at least $1/2+\gamma(n_i)$. Thus $\Ts_i^\Os$ rejects $0^{n_i}$. This means $\Ts_i$ fails to correctly decide $0^{n_i}$.

On the other hand, suppose $x\notin\Language^\Os$. This means that there exists a polynomial-length $w_i$ such that $\Ts_i^{\Os_i}(0^{n_i},w_i)$ accepts with probability at least $1/2+\gamma(n_i)$. We will now show that $\Ts_i^{\Os}(0^{n_i},w_i)$ also accepts with probability strictly more than $1/2+\gamma(n_i)/2$, meaning $\Ts_i^{\Os}$ accepts $x$, and thus meaning $\Ts_i$ fails to correctly decide $0^{n_i}$. This would complete the proof of Theorem~\ref{thm:main}.

Toward accomplishing this goal, we will show that $\Os$ and $\Os_i$ agree on all points that $\Ts_i$ places significant query weight. Consider the procedure that constructed $S'$ by running $\Ts_i^{\Os_i}(0^{n_i},w_i)$ several times, which in turn makes queries to $\Os_i$. Moreover, consider changing this procedure to actually run $\Ts_i^{\Os_i}(0^{n_i},w)$ for a \emph{random} choice of $w$ instead of $w_i$ (the same $w$ is used in all runs of $\Ts_i$). Then the procedure makes $vQ$ queries to $S$, which is in turn sampled from $\Bernoulli_{p}^N$, and $S'$ is always a subset of $S$. It also makes $vQ\leq k/2$ queries to $U$. Recall that while $U$ depends on $S$, $U$ is still $k$-wise uniform independent conditioned on $S$. Therefore, by Lemma~\ref{lem:kwiseindep}, we can conclude the probability of any $S'$ is identical to the case in which $U$ is truly random independent of $S$. But since we can simulate a truly random function without any knowledge of $S$, this means we can simulate the output distribution $S'$ just by making queries to $S$ but not $U$. The algorithm also queries the other parts of $\Os_i$ for inputs of length other than $n$, but $S$ is chosen independently of these other parts of $\Os$. Therefore, by Lemma~\ref{lem:multi}, there is a universal constant $C$ such that $\Pr[|S'|\geq K:w\text{ is uniform}]\leq (Cp(vQ/K)^2)^K$. Since $w=w_i$ with probability  $2^{-q(n_i)}$, we therefore have that $\Pr[|S'|\geq K:w=w_i]\leq 2^{q(n_i)}(Cp(vQ/K)^2)^K$. If we set $K=v Q\sqrt{2 C p} + q(n_i)+\log_2(v)$, we can bound $\Pr[|S'|\geq K:w=w_i]\leq 2^{-v}$. Then in particular since $|S'|\leq v$ always, we have that $\E[|S'|]\leq K$.

Let $e_j$ denote the probability that the $j$th iteration of the loop constructing $S'$ adds an element to $S'$. Then $\sum_{j=1}^v e_j=\E[|S'|]\leq K$. We also have that the $e_j$ are monotonically increasing, since their distributions over $y$ are identical and it only gets harder to output a $y$ not in $S'$ as $S'$ grows. Therefore, we must have that $e_v\leq K/v$. Recall that, among points in the support of queries of $\Ts_i$, $\Os$ and $\Os_i$ agree except on queries to $S_i$, where $\Os_i$ answers with $S$ and $\Os$ answers with $S'$. For an input $y\in S$, let $M_y$ denote the total magnitude squared of $y$ in all queries made by $\Ts_i^{\Os_i}(0^{n_i},w_i)$. Then measuring a random choice of the $\leq Q$ queries by $\Ts_i^{\Os_i}$, we will obtain $y$ with probability at least $M_y/Q$. Since $e_v\leq K/v$, this means that by the end of the loop, the expected total query weight of all points in $S$ but not in $S'$ is at most $QK/v$. By Markov's inequality, we therefore have that the query weight of points in $S\setminus S'$ is at most $\sqrt{QK/v}$, except with probability at most $\sqrt{QK/v}$. Recall that $\sqrt{QK/v}$ is negligible. Therefore, since this probability is negligible, we will therefore assume the total query weight of points in $S\setminus S'$ is at most $\sqrt{QK/v}$.

We now invoke Lemma~\ref{lem:BBBV} to see that the difference in acceptance probability between $\Ts_i^{\Os_i}(0^{n_i},w_i)$ and $\Ts_i^{\Os}(0^{n_i},w_i)$ is at most $4\sqrt{Q\times \sqrt{QK/v}}=4\sqrt[4]{Q^3K/v}$. Observe that $Q^3K/v = Q^4\sqrt{2Cp}+Q^3(q+\log_2(v))/v$. Using that $Q\ll \gamma p^{-1/2}$ and $v\gg qQ^4/\gamma^4$, we therefore have that $Q^3K/v\leq \gamma(n_i)^4/(12)^4$. Hence the difference in acceptance probability is at most $\gamma(n_i)/3$, and hence $\Pr[\Ts_i^{\Os}(0^{n_i},w_i)=1]> 1/2+\gamma(n_i)/2$, as desired.



Analogously to the proof that $\Language^\Os\in\QMA$, for each $n_i$ the above may fail to construct $\Os,\Language^\Os$ such that $\Ts_i$ actually correctly decides if $0^{n_i}\in\Language^\Os$, meaning we fail to show that $\Language^\Os\notin\QCMA^\Os$. However, we showed that the probability for any particular $n_i$ is negligible. As before, we can choose $n_1$ large enough to ensure that the probability of failure among \emph{any} $n_i$ is at most $1/3$.


Taken together, since $\Pr[\Language^\Os\notin\QMA^\Os]\leq 1/3$ and $\Pr[\Language^\Os\in\QCMA^\Os]\leq 1/3$, we therefore have that $\Pr[\Language^\Os\in\QMA^\Os\setminus\QCMA^\Os]\geq 1/3$. Thus, we have established the existence of a classical oracle separating $\QMA$ from $\QCMA$.\end{proof}

